Chameleon: Increasing Label-Only Membership Leakage with Adaptive Poisoning

The integration of machine learning (ML) in numerous critical applications introduces a range of privacy concerns for individuals who provide their datasets for model training. One such privacy risk is Membership Inference (MI), in which an attacker seeks to determine whether a particular data sample was included in the training dataset of a model. Current state-of-the-art MI attacks capitalize on access to the model's predicted confidence scores to successfully perform membership inference, and employ data poisoning to further enhance their effectiveness. In this work, we focus on the less explored and more realistic label-only setting, where the model provides only the predicted label on a queried sample. We show that existing label-only MI attacks are ineffective at inferring membership in the low False Positive Rate (FPR) regime. To address this challenge, we propose a new attack Chameleon that leverages a novel adaptive data poisoning strategy and an efficient query selection method to achieve significantly more accurate membership inference than existing label-only attacks, especially at low FPRs.

==> backup_analysis.tex <==
\subsection{MI Analysis under poisoning} \label{apdx:MIAnalysis}

Let $\dist$ denote the distribution from which $n$ samples $z_1,\ldots,z_n$ are sampled in an iid manner. For classification based tasks, a sample is defined as  $z_i = (x_i,y_i)$ where $x_i$ denotes the input vector and $y_i$ denotes the class label. We assume binary membership inference variables $m_1, \ldots, m_n$ that are drawn independently with probability $\Pr(m_i = 1) = \beta$, where samples with $m_i = 1$ are a part of the training set. 
We assume that the training algorithm introduces randomness while training the  model and the posterior distribution over the model parameters $\theta| z_1,\ldots,z_n,m_1, \ldots, m_n$ can be modeled as:
\begin{align} \label{eqn:postdist}
    \Pr(\theta| z_1,\ldots,z_n,m_1,\ldots,m_n) \propto e^{-\frac{1}{\tau} \sum_{i=1}^n m_i L(\theta, z_i)}
\end{align}
where $\tau$ and $L$ denote the temperature parameter and the loss term respectively. This assumption on the posterior distribution of the model parameters have also been made in previous membership inference papers such as  Sablayrolles et al... We assume prior on $\theta$ to be uniform.

Without loss of generality, let us analyze the case of $z_1 = (x_1, y_1)$, for a binary classification task.  We introduce poisoning by creating a poisoned dataset $\psndata$ which contains $k$ poisoned replicas of $z^p_1 = (x_1, y^p_1)$, where $y^p_1 \neq y_1$. The posterior in Eqn.\ref{eqn:postdist} can then be re-written as:
\begin{align} \label{eqn:psndist}
    \Pr(\theta_p| z_1,\ldots,z_n,m_1,\ldots,m_n,\psndata) \propto e^{-\frac{1}{\tau} \sum_{i=1}^n m_i L(\theta_p, z_i) - \frac{k}{\tau}L(\theta_p, z_1^p)} 
\end{align}

Furthermore, we gather information about other samples and their memberships  in set $T = \{z_2,\ldots,z_n,m_2,\ldots,m_n\}$. We assume the loss function $L$ to be a 0-1 loss function, so that we can bound the total loss in Eqn.$\ref{eqn:psndist}$. 

We  are interested in  determining the probability of selecting a poisoned parameter $\theta_p$ that correctly classifies $z_1$ as $y_1$. We denote this event as  $\theta_p(z_1) = y_1$. Similarly, $\theta_p(z_1) = y^p_1$ represents the selection of a $\theta_p$ that results in misclassification of $z_1$ as $y^p_1$. Let us first consider the OUT case when $z_1$ is not a part of the training set, i.e. $m_1 = 0$.  Formally we can write the probability of selecting a parameter that leads to a correct classification as:  
%
\begin{equation*}
\Pr(\theta_p(z_1) =y_1 | z_1,m_1= 0,T,\psndata)
\end{equation*}
%
Finally, we assume that under the presence of poisoning, the model parameter selection for  classification of $z_1$ depends only on $z_1$, $m_1$ and $\psndata$, i.e. 
%
\begin{equation} \label{eqn:mem}
\Pr(\theta_p(z_1) = y_1 | z_1,m_1= 0,T,\psndata) = \Pr(\theta_p(z_1) = y_1 | z_1,m_1= 0,\psndata)
\end{equation}
%
Subsequently, we can use Eqn.\ref{eqn:psndist} to reformulate Eqn.\ref{eqn:mem} as follows:
%
\begin{align}\label{eqn:outdist} 
\Pr(\theta_p(z_1) = y_1 | z_1,m_1= 0,\psndata) = \frac{e^{-k/\tau}}{e^0 + e^{-k/\tau}} = \sigma\left(-\frac{k}{\tau}\right)
\end{align}
%
where, $\sigma(x) = 1/(1+e^{-x})$ denotes the sigmoid function. In this equation, the numerator $e^{-k/\tau}$ denotes the scenario where a parameter is chosen resulting in correct classification. Similarly, the term $e^{0}$ in the denominator represents the scenario where a parameter is selected that classifies $z_1$ as $y_1^p$.

Similar to Eqn.\ref{eqn:outdist}, we can formulate an equation for the IN case where $z_1$ is in the training set: 
%
\begin{align}
\Pr(\theta_p(z_1) = y_1 | z_1,m_1= 1,\psndata) =  \frac{e^{-k/\tau}}{e^{-1/\tau} + e^{-k/\tau}} = \sigma\left(\frac{1-k}{\tau}\right)
\end{align}

The term $e^{-1/\tau}$ in the denominator denotes the contribution of the original sample $z_1$ in the training set for the missclassification scenario.

\subsubsection{TPR at x\% FPR:}
Under this modelling assumption, given a fixed FPR of $x\%$, we now analyze how the TPR changes by varying the number of poisoned replicas $k$. We say $z_1$ is "IN" the training set if $\theta(z_1) = y_1$, else we say "OUT". The FPR can then be written as

\begin{align*} 
\Pr(\text{ "IN" }| ~\theta_p(z_1) = y_1,z_1,m_1 = 0, \psndata) = \frac{x}{100}
\end{align*}
We can re-write the above equation as:

\begin{align} \label{eqn:fpr}
\Pr(\text{ "IN" }| ~\theta_p(z_1) = y_1) = \frac{0.01 \times x}{\Pr(\theta_p(z_1) = y_1 | z_1,m_1= 0,\psndata)} = \frac{0.01 \times x}{\sigma\left(-\frac{k}{\tau}\right)}
\end{align}

We can then write the TPR as:
\begin{flalign} \label{eqn:tpr}
\nonumber &= \Pr(\text{ "IN" }| ~\theta_p(z_1) = y_1,z_1,m_1 = 1, \psndata) 
\\\nonumber  &= \Pr(\text{ "IN" }| ~\theta_p(z_1) = y_1)
\times \Pr(\theta_p(z_1) = y_1 | z_1,m_1= 1,\psndata)
\\ &=  \frac{0.01 \times x}{\sigma\left(-\frac{k}{\tau}\right)} \times \sigma\left(\frac{1-k}{\tau}\right)
\end{flalign}

\begin{wrapfigure}{r}{0.33\textwidth} %this figure will be at the right
    \centering
    \vspace{-5mm}
    \includegraphics[width=0.33\textwidth]{Figures/TPRBehavior.png}
    \caption{Impact of poisoning on the TPR (@1\% FPR) within our theoretical model for a binary classification task.}
    \vspace{-12mm}
    \label{fig:TPRbehavior}
\end{wrapfigure}
We now plot the TPR as a function of the number of poisoned replicas using Eqn.\ref{eqn:tpr}. We set the temperature parameter $\tau  = 0.5$ and fix the FPR to $1\%$. In Figure \ref{fig:TPRbehavior} we observe that the TPR improves with increase in the number of poisoned replicas.  However, beyond a certain threshold, the TPR improvement becomes marginal, signifying that the most of the improvement occurs with a relatively small amount of poisoning. This provides us with the insight that poisoning can indeed help in improving the TPR metric at a fixed FPR value.


\subsubsection{Multi-class classification Scenario}
We now extend our analysis for the multi-class classification scenario.  Let the total number of classes be $c$. Without of loss of generality let us consider the case of sample $z_1 = (x_1, y_1)$. We use the same poisoning strategy as before where poisoned dataset $\psndata$ contains $k$ poisoned replicas of $z^p_1 = (x_1, y^p_1)$, where $y^p_1 \neq y_1$. Note that, all poisoned replicas have the same poisoned label $y^p_1$. 

We can now write the probability of selecting a model parameter that leads to a correct classification in the OUT case as follows:

\begin{align}\label{eqn:outmultdist} 
\Pr(\theta_p(z_1) = y_1 | z_1,m_1= 0,\psndata) = \frac{e^{-k/\tau}}{e^0 + (c-1) e^{-k/\tau}} = \alpha_{\text{out}}
\end{align}

The term $e^{-k/\tau}$ in the numerator represents the outcome where a parameter is selected that classifies $z_1$ as the true label $y_1$.
The terms $e^0$ and $(c-1)e^{-k/\tau}$ in the denominator represents the outcome where a parameter is selected such that it classifies $z_1$ as $y_1^p$ and any other label except $y_1^p$ respectively.

Similar to Eqn.\ref{eqn:outmultdist}, we can formulate an equation for the IN case as follows:

\begin{align}\label{eqn:inmultdist} 
\Pr(\theta_p(z_1) = y_1 | z_1,m_1= 1,\psndata) = \frac{e^{-k/\tau}}{e^{-1/\tau} + e^{-k/\tau} + (c-2) e^{-(k+1)/\tau}} = \alpha_{\text{in}}
\end{align}

The terms $e^{-1/\tau}$ and $e^{-k/\tau}$ in the denominator represent the outcomes when sample $z_1$ is classified as $y_1^p$ and $y_1$ respectively. Term $(c-2) e^{-(k+1)/\tau}$ denotes the sum over all outcomes where sample $z_1$ is classified as a label except $y_1$ and $ y_1^p$.

\paragraph{TPR at x\% FPR} 
We can formulate an equation for TPR similar to equation \ref{eqn:tpr}  in the binary classification scenario as: 

\begin{flalign} \label{eqn:multtpr}
\Pr(\text{ "IN" }| ~\theta_p(z_1) = y_1,z_1,m_1 = 1, \psndata) =  \frac{0.01 \times x \times \alpha_{\text{in}}}{\alpha_{\text{out}}}
\end{flalign}

\begin{wrapfigure}{r}{0.33\textwidth} %this figure will be at the right
    \centering
    \vspace{-5mm}
    \includegraphics[width=0.33\textwidth]{Figures/MultTPRBehavior.png}
    \caption{Impact of poisoning on the TPR (@1\% FPR) within our theoretical model for a 10-class classification task.}
    \vspace{-10mm}
    \label{fig:multTPRbehavior}
\end{wrapfigure}

We can now plot the TPR as a function of the number of poisoned replicas for the multi-class classification setting using Eqn.\ref{eqn:multtpr}. We set the temperature parameter $\tau  = 0.4$ and the number of classes $c = 10$. We fix the FPR to $1\%$ and observe a similar behavior in the TPR even for the multiclass setting where the TPR improves with increase in poisoning rate. Note that, assigning the number of classes $c$ to 2,  which corresponds to a binary classification task, Eqn.\ref{eqn:multtpr} simplifies to Eqn.\ref{eqn:tpr}, demonstrating that Eqn.\ref{eqn:multtpr} is a generalized form encompassing binary and multi-class scenarios.


\subsubsection{Multi-label Poisoning}
Another potential poisoning strategy in the multi-class scenario could be is to assign a different poisoned label  to each of the $k$ poisoned replica when constructing $\psndata$. Previous works \citep{TruthSerum,MIPoison22} have empirically shown that this strategy of poison does not work as well as the the label-consistent poisoning strategy, where all poisoned replicas of $z_1^p$ have the same poisoned label.
We will now show using our theoretical model on why this multi-label poisoning strategy is not as effective as label-consistent strategy.










==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

